Unrolled Architectures for High-Throughput Encoding of Multi-Kernel Polar Codes

Over the past decade, polar codes have received significant traction and have been selected as the coding method for the control channel in fifth-generation (5G) wireless communication systems. However, conventional polar codes are reliant solely on binary (2x2) kernels, which restricts their block length to being only powers of 2. In response, multi-kernel (MK) polar codes have been proposed as a viable solution to attain greater code length flexibility. This paper proposes an unrolled architecture for encoding both systematic and non-systematic MK polar codes, capable of high-throughput encoding of codes constructed with binary, ternary (3x3), or binary-ternary mixed kernels. The proposed scheme exhibits an unprecedented level of flexibility by supporting 83 different codes and offering various architectures that provide trade-offs between throughput and resource consumption. The FPGA implementation results demonstrate that a partially-pipelined polar encoder of size N=4096 operating at a frequency of 270 MHz gives a throughput of 1080 Gbps. Additionally, a new compiler implemented in Python is given to automatically generate HDL modules for the desired encoders. By inserting the desired parameters, a designer can simply obtain all the necessary VHDL files for FPGA implementation.

==> BU.tex <==
\begin{table*}
\centering
\caption{Post-fitting results of various Combinational MK polar Encoders}
\begin{tabular}{cccccccc}
\hline
\begin{tabular}[c]{@{}c@{}}Block \\Length  \end{tabular}  &Kernel Order& LUTs  & Reg. & \begin{tabular}[c]{@{}c@{}}RAM \\(bits)  \end{tabular} &
\begin{tabular}[c]{@{}c@{}}L \\($\mu$s)  \end{tabular}&
\begin{tabular}[c]{@{}c@{}}f \\(MHz)  \end{tabular}&
\begin{tabular}[c]{@{}c@{}}T/P \\(Gbps) \end{tabular}\\\hline
192&\{3,2,2,2,2,2,2\}     & 530 &  1091 & 0 & 1 & 166 & 31.125\\%31.872Mbps
256&\{2,2,2,2,2,2,2,2\}   & 616 & 1411 & 0 &1 & 159&39.75 \\%40.704 Mbps
243&\{3,3,3,3,3\}         & 675 & 1346  & 0 &1& 178 & 42.24 \\%43.254Mbps
324&\{2,2,3,3,3,3\}       & 918 & 1752 & 0 &1& 117 & 37.02 \\%37,908Mbps
384&\{3,2,2,2,2,2,2,2\}   & 1127 & 2052 & 0 &1& 108 & 40.5 \\%41.472Mbps
512&\{2,2,2,2,2,2,2,2,2\} & 1397 & 2692 & 0 &1 & 75&37.5 \\%38.4Mbps
576&\{2,2,2,2,2,2,3,3\}   & 1547 & 3013 & 0 &1 & 61 & 34.312 \\%35,136Mbps
%729&\{3,3,3,3,3,3\}       &  &  & 0 & &   &  \\%Mbps
%768&\{2,2,3,2,2,2,2,2,2\} &  &  & 0 &&   & \\%Mbps
1024&\{2,2,2,2,2,2,2,2,2,2\} & 2965 & 5253 & 0 &1 & 36.5&36.5\\%37.376Mbps
%1536& \{3,2,2,2,2\}         &  &   & 0 & & &  \\ %Mbps
%1728&\{3,3,3,3\}            &  &   & 0 & & &    \\ %Mbps
%2048&\{2,2,2,2,2,2,2,2,2,2,2\} & 6628 & 10293 & 0 &1 & 6.64&13.6 \\%850/16 128
2048&\{2,2,2,2,2,2,2,2,2,2,2\} & 6533 & 10383 & 0 &1 & 16&  32\\%32.768Mbps
%2916&\{3,2,2,2,2,2,2\}     &  &   & 0 & & &  \\ 
%3888&\{3,3,3,3,3\}         &  &   & 0 & & & \\ 
%768&\{2,2,3,2,2,2,2,2,2\} & 2442 & 3883 & 0 &1 & 16.15&12.4 && & & \\     %775/48
%4096&\{2,2,2,2,2,2,2,2,2,2,2,2\} & 13851 & 20548 & 0 &1 &3.03 &12.4 \\%775/256
\hline
\end{tabular}
\label{tab:MKEnc}
\end{table*}




\begin{table*}
\centering
\caption{Post-fitting results of various Combinational MK polar Encoders}
\begin{tabular}{cccccccc}
\hline
\begin{tabular}[c]{@{}c@{}}Block \\Length  \end{tabular}  &Kernel Order& LUTs  & Reg. & 
\begin{tabular}[c]{@{}c@{}}L \\(CCs)  \end{tabular}&
\begin{tabular}[c]{@{}c@{}}L \\($\mu$s)  \end{tabular}&
\begin{tabular}[c]{@{}c@{}}f \\(MHz)  \end{tabular}&
\begin{tabular}[c]{@{}c@{}}T/P \\(Gbps) \end{tabular}\\\hline
\hl{128}&\{2,2,2,2,2,2,2\}& 260 & 384 & 1 &0.0028 & 352&44\\
192&\{3,2,2,2,2,2,2\}     & 530 &  1091 & 1 & 1 & 166 & 31.125\\%31.872Mbps
\hl{256}&\{2,2,2,2,2,2,2,2\}   & 552 & 512 & 1 & &270 &67.5\\%40.704 Mbps419/4
243&\{3,3,3,3,3\}         & 675 & 1346  & 1 &1& 178 & 42.24 \\%43.254Mbps
324&\{2,2,3,3,3,3\}       & 918 & 1752 & 1 &1& 117 & 37.02 \\%37,908Mbps
384&\{3,2,2,2,2,2,2,2\}   & 1127 & 2052 & 1 &1& 108 & 40.5 \\%41.472Mbps
512&\{2,2,2,2,2,2,2,2,2\} & 1397 & 2692 & 1 &1 & 75&37.5 \\%38.4Mbps
576&\{2,2,2,2,2,2,3,3\}   & 1547 & 3013 & 1 &1 & 61 & 34.312 \\%35,136Mbps
%729&\{3,3,3,3,3,3\}       &  &  & 0 & &   &  \\%Mbps
%768&\{2,2,3,2,2,2,2,2,2\} &  &  & 0 &&   & \\%Mbps
1024&\{2,2,2,2,2,2,2,2,2,2\} & 2965 & 5253 & 1 &1 & 36.5&36.5\\%37.376Mbps
%1536& \{3,2,2,2,2\}         &  &   & 0 & & &  \\ %Mbps
%1728&\{3,3,3,3\}            &  &   & 0 & & &    \\ %Mbps
%2048&\{2,2,2,2,2,2,2,2,2,2,2\} & 6628 & 10293 & 0 &1 & 6.64&13.6 \\%850/16 128
%2048&\{2,2,2,2,2,2,2,2,2,2,2\} & 6533 & 10383 & 0 &1 & 16&  32\\%32.768Mbps
%2916&\{3,2,2,2,2,2,2\}     &  &   & 0 & & &  \\ 
%3888&\{3,3,3,3,3\}         &  &   & 0 & & & \\ 
%768&\{2,2,3,2,2,2,2,2,2\} & 2442 & 3883 & 0 &1 & 16.15&12.4 && & & \\     %775/48
%4096&\{2,2,2,2,2,2,2,2,2,2,2,2\} & 13851 & 20548 & 0 &1 &3.03 &12.4 \\%775/256
\hline
\end{tabular}
\label{tab:MKEnc}
\end{table*}
